An Empirical Study on Strong-Weak Model Collaboration for Repo-level Code Generation

We study cost-efficient collaboration between strong and weak language models for repository-level code generation, where the weak model handles simpler tasks at lower cost, and the most challenging tasks are delegated to the strong model. While many works propose architectures for this task, few analyze performance relative to cost. We evaluate a broad spectrum of collaboration strategies: context-based, pipeline-based, and dynamic, on GitHub issue resolution. Our most effective collaborative strategy achieves equivalent performance to the strong model while reducing the cost by 40%. Based on our findings, we offer actionable guidelines for choosing collaboration strategies under varying budget and performance constraints. Our results show that strong-weak collaboration substantially boosts the weak model's performance at a fraction of the cost, pipeline and context-based methods being most efficient. We release the code for our work at https://github.com/shubhamrgandhi/codegen-strong-weak-collab.

==> sections/background.tex <==


% \section{Preliminary}

% \subsection{Repository-Level Code Generation with SWE-Bench} \label{sec:swebench}

% Repository-level code generation is an up and coming problem to be tackled by LLMs. The SWE-bench benchmark is specifically designed to evaluate models on software engineering tasks derived from real-world GitHub issues. Each task consists of an issue description with the goal of generating a patch that resolves that issue i.e. passes a certain set of tests. Unlike traditional function-level or file-level code generation tasks, SWE-Bench considers repository-level context and requires models to reason at a codebase-level rather than isolated code snippets. These properties make SWE-Bench a challenging task for studying cost-effective techniques for knowledge transfer and collaboration between strong and weak LLMs for code. In this work, we focus on the SWE-Bench Lite \footnote{\url{https://www.swebench.com/lite.html}} subset, which has 300 test instances spanning across 12 repositories. It is a simpler version of the full SWE-Bench in the sense that it does \textit{not} have instances where the ground truth patch has more than 3 edit hunks and spans across multiple files, apart from other selection criteria. 


% \subsection{Agentless Lite Framework}
% This reflects the standard RACG pipeline where all retrieved files and the input are concatenated into a single prompt for generation.


% \yiqing{TBD: explain that we choose RACG, not agentic frameworks or even Agentless because it is significantly more cost-efficient (show some numbers here) and aligns better with our ultimate goal of reducing cost. In principle, our strong-weak collaboration methods can also be applied to other frameworks.} \shubham{Added}

% We perform this study with Agentless Lite, an RACG pipeline described in Appendix \ref{sec:agentless_lite}, since it is inherently cost-efficient and costs ~91\% less than agentic methods like SWE-Agent, or even ~70\% less than Agentless.
% However, in principle, our strong-weak LM collaboration methods can also be applied to other frameworks.

% To perform our experiments, we adopt the Agentless Lite \footnote{\url{https://github.com/sorendunn/Agentless-Lite}} framework, a recent RAG + Code-gen style scaffold designed for complex coding tasks. It is a lightweight adaptation of the Agentless Framework \cite{agentless}. Agentless Lite follows a two-step approach: (1) retrieve the top \(k\) relevant files using a pretrained embedding model, and (2) use a language model to generate a candidate patch based on the retrieved context and issue problem statement. Agentless Lite is model-agnostic, inference-only, and does not require a sandboxed runtime environment. This makes it suitable for rapid evaluation across multiple strategies.


==> sections/introduction_v1.tex <==
\section{Introduction}
\label{sec:introduction}

% Key idea - We aim to study the types of information a strong agent can provide to a weak agent that are both effective and cost-efficient.

% Motivate the problem: repo-level code generation.

% Motivate Strong-Weak collaboration. 
% Motivate empirical study (why will people find this useful??)
% Briefly mention related work. What's lacking (no systematic analysis)

% In this paper, we present a taxonomy of strong-weak collaboration methods, ... 
% (why is this taxonomy relatively comprehensive? How/Why do we choose these methods?)

% One or two lines introducing the experiment setup. (probably briefly mention here that we prioritize pipeline-based methods because they are cost-efficient. In principle, our methods can also be applied to agentic frameworks.)
% Empirical results. 
% Highlight interesting findings: 
% 1, the best methods give XX performance gain over 4o-mini and Qwen-7B. Mention the numbers here.
% 2, 3, ...


Recent progress in Large Language Models (LLMs) has enabled notable capabilities for repository-level (repo-level) code generation, which aims to solve real-world coding problems in naturally occurring repositories.
% and demands both the understanding of repo-level information and the capabilities to solve complicated coding problems~\cite{jimenez2024swebench,zhang-etal-2023-repocoder}.
% \yiqing{TBD: introduce RAG-for-code here: use one sentence to describe what it is and say that it is a standard setting (cite CodeRAGBench), and then use another sentence to motivate RAG-for-code)}
% \shubham{Added}
Retrieval-Augmented Code Generation (RACG) has emerged as a standard and effective setting for tackling such tasks~\cite{wang-etal-2025-coderag}. It involves first retrieving relevant files from the repository and then passing them as context to an LLM. This setting is particularly appealing due to its modularity and cost-efficiency, as it allows the model to focus generation efforts on a narrowed, context-rich subset of code rather than processing the entire repository.
Empirical results~\cite{agentless,wang-etal-2025-coderag} show that relatively weak models still struggle to independently solve such complex, multi-step tasks, while solely relying on strong models typically requires a very steep cost (e.g., API cost). 


A natural question to ask is: can strong and weak models collaborate in a way that is both effective and cost-efficient?
Prior work has explored strong-weak collaboration ideas for traditional NLP tasks, including chain-of-thought distillation \cite{magister2023teachingsmalllanguagemodels, ranaldi-freitas-2024-aligning}, model cascades \cite{chen2023frugalgptuselargelanguage}, context augmentation \cite{chen2025codesteersymbolicaugmentedlanguagemodels}, etc. 
However, to our knowledge, there is no systematic empirical analysis of strong-weak collaboration in the code generation domain, which could potentially guide future deployments of code generation frameworks, especially when cost, latency, and compute resources are major considerations.

% Prior work has explored strong-weak collaboration ideas in related settings such as chain-of-thought distillation \cite{magister2023teachingsmalllanguagemodels, ranaldi-freitas-2024-aligning} and model cascades for cost efficiency \cite{chen2023frugalgptuselargelanguage} along with techniques such as self-consistency \cite{wang2023selfconsistencyimproveschainthought, chen2023universalselfconsistencylargelanguage} to improve standalone weak LM performance with increased budget. However, to our knowledge, there is no systematic taxonomy or empirical comparison focused specifically on strong-weak collaboration for repository-level code tasks.

% In this paper, we undertake an empirical study to systematically investigate how strong models can assist weak models in a cost-efficient manner for repository-level code generation. We believe such a study is critical for future deployments of LLM agents in real-world coding environments, where cost, latency, and compute resources are major considerations.

To bridge this gap, in this paper, we conduct an empirical study to systematically investigate how strong models and weak models can collaborate in repo-level code generation.
\yiqing{We focus on the RAG-for-code setting due to its inherent cost-efficiency compared to agentic frameworks (probably cite some numbers here).} \shubham{Added one line} We focus on the RAG-for-code setting due to its inherent cost-efficiency compared to agentic frameworks, with previous works stating that RAG can be up to 99\% cheaper \cite{jin2025llmsllmbasedagentssoftware}.
As shown in Figure \ref{fig:taxonomy}, we present a three-layer taxonomy containing 12 diverse collaboration methods between strong and weak LLMs, ranging from static context injection (e.g., few-shot examples, FAQs, Planning), pipeline division (e.g., prompt reduction, fallback), and dynamic collaboration (e.g., via routing). 
Then we implement and test those 12 methods for the collaboration between two API-based models and between one API-based and one open-source model on the SWE-Bench~\cite{jimenez2024swebench} dataset.
% We also benchmark cost-equated single model baselines to motivate the effectiveness of collaboration.

% We conduct experiments using the Agentless Lite framework, a retrieval-augmented code generation system. While we prioritize such a pipeline-based system due to ease of experimentation and inherent cost-efficiency, our studied approaches can also be extended to more complex agentic settings involving dynamic multi-turn strong LM-weak LM interaction.

Our empirical results demonstrate that strong-weak collaboration can significantly improve weak LM performance in a cost-efficient manner. For instance, the best collaboration methods yield up to a xx\% improvement for Qwen2.5-Coder-7B and a xx\% improvement for GPT-4o-mini, compared to their base performance. 
We further conduct detailed analyses of the results. Our main findings include: ... 
\shubham{insert findings here.} 
% These findings suggest that carefully designed collaboration strategies can significantly bridge the gap between strong LMs and weak LMs without incurring a substantial cost overhead. 
Overall, this study provides a foundation for designing future cost-efficient, collaborative LLM systems for complex code generation tasks.

==> sections/introduction_v2.tex <==
\section{Introduction}
\label{sec:introduction}

% Key idea - We aim to study the types of information a strong agent can provide to a weak agent that are both effective and cost-efficient.

% Motivate the problem: repo-level code generation.

% Motivate Strong-Weak collaboration. 
% Motivate empirical study (why will people find this useful??)
% Briefly mention related work. What's lacking (no systematic analysis)

% In this paper, we present a taxonomy of strong-weak collaboration methods, ... 
% (why is this taxonomy relatively comprehensive? How/Why do we choose these methods?)

% One or two lines introducing the experiment setup. (probably briefly mention here that we prioritize pipeline-based methods because they are cost-efficient. In principle, our methods can also be applied to agentic frameworks.)
% Empirical results. 
% Highlight interesting findings: 
% 1, the best methods give XX performance gain over 4o-mini and Qwen-7B. Mention the numbers here.
% 2, 3, ...

Recent advances in large language models (LLMs) have demonstrated impressive capabilities across complex reasoning and generation tasks. However, benchmark gains are often prioritized over practical deployment concerns, leading to systems that rely on repeated calls to expensive proprietary LLMs. 
For example, SWE-Agent \cite{yang2024sweagentagentcomputerinterfacesenable} caps each run at \$4, with many executions involving hundreds of thousands of tokens~\cite{kapoor2024aiagentsmatter}, making even modest-scale evaluations prohibitively expensive.
\shubham{Can remove the example if it takes up too much space}
In contrast, non-agentic systems such as Retrieval-Augmented Generation (RAG) have been shown to be substantially more efficient. Prior work suggests that RAG-based pipelines can be up to 99\% cheaper than their agentic counterparts~\cite{jin2025llmsllmbasedagentssoftware}.

This motivates a critical question: how can we design LLM systems that are not only effective but also cost-efficient? One promising direction lies in modular, retrieval-augmented pipelines that minimize wasteful computation and restrict model calls to only the most relevant contexts. Retrieval-Augmented Code Generation (RACG)~\cite{wang-etal-2025-coderag} is a well-established framework in this space. Rather than prompting an LLM with the entire problem context, RACG first retrieves relevant code snippets and then passes them into the model. Recent works like Agentless~\cite{agentless} and Agentless Lite~\cite{AgentlessLite2025} have shown that such pipelines can resolve repository-level tasks at a fraction of the cost, with Agentless Lite resolving issues at an average cost of \$0.25. 
% \shubham{Should I add something like this - For the remainder of this paper, we stick to Agentless Lite as the architecture due to its inherent cost-efficient nature.}
% \atharva{No I think this is good enough, since we have limited real estate on a short paper, the most relevant example (Agentless-lite in this case) is good enough}


% \atharva{The paragraph below is rather abrupt. How did we transition from discussing RACG is better than code agents to a weak and a strong model working together? Seems like you need a couple of lines of how you can offload simple tasks to cheaper and weaker models that are capable of doing them. Currently you are building up to an argument that RAG > Agents} \shubham{Added}

While RACG pipelines substantially reduce cost, many real-world code generation tasks vary in complexity. Simple tasks can often be resolved by cheaper, smaller models, whereas more complex problems demand the reasoning capabilities of stronger LMs. This naturally motivates hybrid systems that offload simple tasks to weak models and escalate harder ones to strong models.
However, designing such hybrid systems is non-trivial: weak models alone often fail to solve complex tasks, while relying solely on strong models undermines the cost savings introduced by RACG. This sets the stage for a hybrid question: \textit{Can strong and weak models collaborate in a way that is both effective and cost-conscious?}

% Nonetheless, the challenge remains: weak models alone often fail to solve complex tasks, while relying solely on strong models undermines the cost savings introduced by RACG. This sets the stage for a hybrid question: \textit{Can strong and weak models collaborate in a way that is both effective and cost-conscious?}
% \atharva{this should be before the `Nonetheless, the challenge remains:` part and should be motivated based on the cost idea.} \shubham{Changed the wording a bit.}
% \atharva{Should we talk about CoT distillation since it is more of a training method and we don't have any training methods} \shubham{removed CoT distillation and replaced with ensembling}
Prior work has explored strong-weak collaboration ideas for traditional NLP tasks, including 
% chain-of-thought distillation \cite{magister2023teachingsmalllanguagemodels, ranaldi-freitas-2024-aligning}, 
model cascades \cite{chen2023frugalgptuselargelanguage, zhang2023ecoassistantusingllmassistant, yue2024largelanguagemodelcascades}, context augmentation \cite{chen2025codesteersymbolicaugmentedlanguagemodels}, ensembling \cite{zhang2024smalllanguagemodelsneed, chen2024improvinglargemodelssmall},  etc. 
However, to our knowledge, there is no systematic empirical analysis of strong-weak collaboration in the code generation domain, which could potentially guide future deployments of code generation frameworks, especially when cost is a major consideration.

% Recent progress in Large Language Models (LLMs) has enabled notable capabilities for repository-level (repo-level) code generation, which aims to solve real-world coding problems in naturally occurring repositories.
% and demands both the understanding of repo-level information and the capabilities to solve complicated coding problems~\cite{jimenez2024swebench,zhang-etal-2023-repocoder}.
% \yiqing{TBD: introduce RAG-for-code here: use one sentence to describe what it is and say that it is a standard setting (cite CodeRAGBench), and then use another sentence to motivate RAG-for-code)}
% \shubham{Added}
% Retrieval-Augmented Code Generation (RACG) has emerged as a standard and effective setting for tackling such tasks~\cite{wang-etal-2025-coderag}. It involves first retrieving relevant files from the repository and then passing them as context to an LLM. This setting is particularly appealing due to its modularity and cost-efficiency, as it allows the model to focus generation efforts on a narrowed, context-rich subset of code rather than processing the entire repository.
% Empirical results~\cite{agentless,wang-etal-2025-coderag} show that relatively weak models still struggle to independently solve such complex, multi-step tasks, while solely relying on strong models typically requires a very steep cost (e.g., API cost). 

% A natural question to ask is: can strong and weak models collaborate in a way that is both effective and cost-efficient?


% Prior work has explored strong-weak collaboration ideas in related settings such as chain-of-thought distillation \cite{magister2023teachingsmalllanguagemodels, ranaldi-freitas-2024-aligning} and model cascades for cost efficiency \cite{chen2023frugalgptuselargelanguage} along with techniques such as self-consistency \cite{wang2023selfconsistencyimproveschainthought, chen2023universalselfconsistencylargelanguage} to improve standalone weak LM performance with increased budget. However, to our knowledge, there is no systematic taxonomy or empirical comparison focused specifically on strong-weak collaboration for repository-level code tasks.

To bridge this gap, we conduct an empirical study to systematically investigate how strong models and weak models can collaborate in repo-level code generation.
% \yiqing{We focus on the RAG-for-code setting due to its inherent cost-efficiency compared to agentic frameworks (probably cite some numbers here).} \shubham{Added one line} 
% We focus on the RAG-for-code setting due to its inherent cost-efficiency compared to agentic frameworks, with previous works stating that RAG can be up to 99\% cheaper \cite{jin2025llmsllmbasedagentssoftware}.
As shown in Figure \ref{fig:taxonomy}, we present a three-pronged taxonomy containing 12 diverse collaboration methods between strong and weak LLMs, ranging from static context injection (e.g., Few-Shot examples, FAQs, Planning), pipeline division (e.g., Strong LM First, Prompt Reduction), and dynamic collaboration (e.g., Routing). We combine methods drawn from prior literature with several new or adapted strategies tailored for our setting and test these 12 methods for collaboration between two API-based models and between one API-based and one open-source model on the SWE-Bench~\cite{jimenez2024swebench} dataset. 
Our goal is to empirically characterize the cost-performance trade-offs of these methods and identify best practices under different budget and accuracy constraints. While issue-solving serves as a grounded and challenging testbed, our broader focus is on the general design space of strong–weak collaboration.

% We also benchmark cost-equated single model baselines to motivate the effectiveness of collaboration.

% We conduct experiments using the Agentless Lite framework, a retrieval-augmented code generation system. While we prioritize such a pipeline-based system due to ease of experimentation and inherent cost-efficiency, our studied approaches can also be extended to more complex agentic settings involving dynamic multi-turn strong LM-weak LM interaction.

% We evaluate these strategies on various strong-weak model pairs, including 
% O4-mini, O3-mini, GPT-4o-mini, and Qwen2.5-Coder 
% both closed and open-sourced models 
% \atharva{do we really need to mention the model families in the intro} \shubham{I think it would be better to do so, so that we can show that we have a mix of closed and open source models}.
% Our empirical results demonstrate that strong-weak collaboration can significantly improve weak LM performance in a cost-efficient manner. 
Our results reveal consistent patterns across model pairs, wherein pipeline and context-based strategies offer the best average efficiency, while weak-only baselines underperform despite similar cost. Yet, we find that average efficiency does not always predict optimality. Through cost-performance curves, we answer the question - \textit{What is the best method given a performance requirment and budget constraint?}. This underscores the need for adaptive collaboration strategies guided by practical constraints.
Our best collaboration-based methods are able to give a 62\% gain in accuracy over the weak model, almost matching the strong model's performance at just 60\% cost. 
% \shubham{Should I mention 33\% here (Strong LM First for O3-mini + Qwen 32B) or 41\% here (Strong LM First for O4-mini + GPT-4o-mini)}
% Moreover, we present a thorough comparison of performance vs. cost for various strong-weak model pairs, through which we answer the question of \textit{What is the best performing method one can employ given a specific budget?}
% These findings suggest that carefully designed collaboration strategies can significantly bridge the gap between strong LMs and weak LMs without incurring a substantial cost overhead. 
Overall, this study provides a foundation through actionable principles for designing cost-efficient, collaborative LLM systems for complex code generation tasks in the future.
% We conclude with actionable principles for selecting collaboration strategies given a fixed budget and desired accuracy, providing practical guidance for system designers.

==> sections/results_and_analysis.tex <==
% \section{Results and Analysis}

\begin{figure}
    \centering
    \includegraphics[width=1\linewidth]{figures/combined_performance_cost_curves.png}
    \caption{Performance vs. Cost curves for different Strong-Weak Model Pairs. O3 - O3-mini; O4 - O4-mini; 4o - GPT-4o-mini; Qx - Qwen2.5-Coder-xB. We also provide detailed pairwise results in the Appendix section \ref{sec:pairwise_analysis}.}
    \label{fig:combined_perf_vs_cost}
\end{figure}





\subsection{Main Results}
\label{sec:results_and_analysis}

We restrict evaluation of collaboration methods to the generator module of the Agentless Lite pipeline, since the retriever gets close to perfect performance. 
We observe that the Voyage-Code-3 retriever already achieves ~92\% recall and ~76\% MRR for SWEBench-Lite.
Our results reveal clear patterns about when strong–weak collaboration helps and when it falters, detailed results for which can be found in Appendix sections \ref{sec:pairwise_analysis}, \ref{sec:category_wise} and  \ref{sec:localization}. 



% \yiqing{Figures: cost-performance scatter/curve plots (e.g., for each cost, curve the point with the best performance)}

% \yiqing{RQ1: Are there any methods that in general work for all the strong-weak pairs?}

\start{Cost-equated baselines vs. Strong-Weak collaboration}

As shown in figure \ref{fig:combined_perf_vs_cost}, appendix \ref{sec:pairwise_analysis} and figure \ref{fig:perf_cost_comparison}, we can see that in almost all of the Strong-Weak LM pairs, the cost-equated baselines, i.e. sampling multiple times to match the strong LM's cost,
fares significantly lower than the collaborative methods. Moreover, some patch selection methods even cause deterioration in performance when compared to the base weak LM setting. \atharva{This is an interesting claim where we are saying you can end up spending more money for worse performance. I think we need to justify this a bit more or people will feel we glossed over a very shocking result. Maybe talk about the valid patch rate being an imperfect proxy for resolution rate and hence causing this issue}. \shubham{I think we can mention the valid patch rate bit in the limitations? We can say that for the sake of simplicity we consider valid patch rate as a termination criterion, but more complex approaches could involve something more sophisticated as well.}
Our best collaboration setting, Strong LM First, is able to achieve a resolution rate of 0.4167, which is a ~92\% improvement over the best corresponding cost-equated baseline, i.e., best-of-n for GPT-4o-mini cost-equated with O4-mini setting. These results show that purely weak LM-based methods generally fare significantly worse than strong-weak collaborative methods with the same or lower cost.

\start{Efficacy of methods across model pairs and budget regimes.}

Across model pairs and cost regimes, we observe that no single collaboration method consistently dominates. Pipeline-based strategies like Strong LM First and Weak LM First generally perform best for their cost, particularly when the weak model is reasonably capable. In contrast, when the weak model is very underpowered, such as Qwen2.5-Coder-7B, even collaborative setups yield modest gains at best. Dynamic approaches like Weak Router strike a strong cost–performance balance, especially with closed-source weak models like GPT-4o-mini.

The effectiveness of each method also depends heavily on the model pair and budget. For example, Figure \ref{fig:subfig6} shows that Strong LM First with O3-mini and Qwen2.5-Coder-32B achieves nearly the same resolution rate as using O3-mini alone, while costing only 60\% as much. Beyond that point, additional spending delivers little improvement, highlighting the value of targeted collaboration, i.e., using the strong model just enough to offset the weak model’s limitations without overspending. Moreover, figure \ref{fig:combined_perf_vs_cost} shows a shift in optimal configurations around the \$18.3 mark: O3 + Qwen32B dominates below this threshold, while O4 + GPT-4o-mini becomes more effective above it. These trends underscore that \textit{the best strategy depends not only on absolute model strength but also on budget and performance targets}.

% We observe that pipeline-based collaborative methods like Weak LM First and Strong LM First often achieve the best performance for the corresponding cost for a majority of the model pairs, with the exception of cases where the weak model is very weak, i.e. Qwen2.5-Coder-7B. Moreover, with closed-source weak models, we also observe that the weak router setting also achieves the best performance for its cost. In general, we observe that most methods of collaboration do not work out well in cases where the strong LM is relatively weak and there isn't a significant gap between the strong and weak LM's base performance. Interestingly enough, we see that there is no universal model pair that conclusively performs better than the rest. We see that there lies an inflection point around the cost of \$18.3, before which O3-mini + Qwen2.5-Coder-32B has a higher performance for the same cost, and after which O4-mini + GPT-4o-mini fares the best. A more comprehensive analysis can be found in Appendix \ref{sec:pairwise_analysis}.

% \start{What are the performance gains of each strong–weak collaboration method, and are those gains achieved cost-efficiently?}



% \start{What are the common failure modes in repository-level code generation when using strong–weak collaborations, and how do different methods address (or exacerbate) these failures?}



% \start{Are there cases where the collaboration produces “partial” successes (e.g. a patch that is valid but doesn’t resolve the issue), and what does this reveal about calibration and reliability of the methods?} \shubham{Better to not mention this otherwise people would question the choice of patch validity as termination criterion}




% \subsection{Detailed / Qualitative Analysis}


% \start{How do different types of tasks (as categorized by Agentless' taxonomy) respond to strong–weak collaboration, and which problem categories remain challenging?}


\subsection{Interesting cases}

% \shubham{Interesting cases - (1) repo-level context fails across the board, (2) Few shot examples don't work, (3) Weak router is better than strong router, (4) Some methods like prompt reduction result in drastic drop in valid patch rate (and hence increase cost) but still improve resolution rate}

\start{Instance-level help is better than repo-level help}
% \atharva{consider reframing this as instance level context/help is better than repo-level context/help} \shubham{Done}

All static repo-level context methods proved ineffective across model pairs. Techniques like providing a repository summary, high-level structural info, or FAQs consistently failed to improve the weak model’s success rate by any significany amount. We interpret this as evidence that broad high-level context is too abstract to aid in solving specific coding issues. Specifically, the added information likely distracts the weak LM or dilutes the truly relevant file-level details. Similarly, incorporating few-shot examples in the prompt (whether randomly selected issues or semantically similar ones) did not boost performance and instead reduces the weak LM's performance below the base performance. On the other hand, methods under instance-level context, i.e. plan and instance-level QA pairs, were mostly successful across the board. This shows that although such methods are significantly more costly than providing repo-level context, the gain in performance is far greater, thus making such methods generally more efficient.

\start{Weak Router is better than Strong Router.}

A particularly interesting finding is the counter-intuitive performance of our Dynamic Collaboration strategies, where we observe the weak router often outperforming the strong router, both in terms of resolution rate and cost. For instance, we see that in the case with O4-mini as the strong LM and Qwen2.5-Coder-32B as the weak LM, the weak router setting achieves a resolution rate that is 6 percentage points higher, with a 20\% lesser cost. We suspect that this gap might be due to differences in fundamental capabilities of the models we consider as strong or weak. We see that models like O3-mini and O4-mini, inspite of being good at problem solving, end up overthinking when it comes to making decisions like routing \cite{cuadron2025dangeroverthinkingexaminingreasoningaction}. Only in scenarios where the weak model is extremely incapable, such as Qwen2.5-Coder-7B, did we see the strong router edge out slightly in success rate, and even there the gains were marginal, suggesting it’s rarely worth the cost.

\start{Prompt Reduction trades turn-wise validity for overall performance}

Another notable finding involves the Prompt Reduction strategy, which involves using the weak LM first to get rid of irrelevant context before using the strong LM for generation. Surprisingly, this leads to a significantly lower valid patch rate (~65\% as compared to ~95\% on average for other successful methods), increasing the number of retries and inflating cost. Despite this, prompt reduction often yielded better resolution rates than settings with full prompt context. This counterintuitive result suggests that aggressively trimming irrelevant or distracting files can help the model focus on essential components, even if many attempts fail in the process. In effect, prompt reduction trades off per-attempt quality for increased focus, leading to higher success at the cost of efficiency. However, this strategy can be expensive and unreliable when budget is limited or when model validity is highly sensitive to missing context.

% Principles for choosing models / methods given cost and performance constraints. What are our 'actionable' contributions?

==> sections/results_and_analysis_v2.tex <==
% \section{Results and Analysis}

\begin{figure}
    \centering
    \includegraphics[width=1\linewidth]{figures/combined_performance_cost_curves.png}
    \caption{Performance vs. Cost curves for different Strong-Weak Model Pairs. O3 - O3-mini; O4 - O4-mini; 4o - GPT-4o-mini; Qx - Qwen2.5-Coder-xB. Detailed pairwise results in Appendix section \ref{sec:pairwise_analysis}.}
    \label{fig:combined_perf_vs_cost}
\end{figure}





\subsection{Main Results}
\label{sec:results_and_analysis}

We focus our evaluation on the generator module, as retrieval with \texttt{voyage-code-3} achieves near-perfect performance (\textasciitilde
92\% recall, \textasciitilde
76\% MRR).
Our findings uncover consistent patterns in when strong–weak collaboration succeeds or fails (Appendix \ref{sec:pairwise_analysis}-\ref{sec:localization}). 


\start{Cost-equated baselines vs. Strong-Weak collaboration}

As shown in Figure \ref{fig:combined_perf_vs_cost}, Appendix \ref{sec:pairwise_analysis} and Appendix Figure \ref{fig:perf_cost_comparison},across nearly all model pairs, the cost-equated baselines, i.e. sampling multiple times to match the strong LLM's cost, underperform compared to strong-weak collaboration. Surprisingly, some baselines even degrade performance relative to the base weak LLM setting, which is likely due to faltering patch selection.
% Moreover, some patch selection methods even cause deterioration in performance when compared to the base weak LM setting. 
% \atharva{This is an interesting claim where we are saying you can end up spending more money for worse performance. I think we need to justify this a bit more or people will feel we glossed over a very shocking result. Maybe talk about the valid patch rate being an imperfect proxy for resolution rate and hence causing this issue}. 
% \shubham{I think we can mention the valid patch rate bit in the limitations? We can say that for the sake of simplicity we consider valid patch rate as a termination criterion, but more complex approaches could involve something more sophisticated as well.}
Our best collaboration setting, Strong LM First, achieves a 0.4167 resolution rate, which is ~92\% more than the best corresponding cost-equated baseline, i.e., best-of-n for GPT-4o-mini cost-equated with O4-mini setting. 
% These results show that purely weak LM-based methods generally fare significantly worse than strong-weak collaborative methods with the same or lower cost.

\start{Efficacy of Methods Across Taxonomy Groups}

Analyzing by taxonomy (Section~\ref{sec:approach}), on average, pipeline and context-based strategies yield the highest cost-efficiency across model pairs, followed by dynamic methods and \textit{Best of n}, with self-consistency approaches being the lease efficient (Appendix~\ref{sec:stats}).

However, average efficiency alone is not enough to identify the best strategy. As shown in Figure~\ref{fig:combined_perf_vs_cost}, cost–performance curves for different methods frequently intersect. For instance, \underline{Weak LM First} is often optimal in low-budget settings due to its minimal strong LM usage. As the budget increases, \underline{Strong LM First} becomes dominant, achieving performance close to that of the standalone strong model at around 60\% of the cost. Figure~\ref{fig:subfig6} illustrates this with O3-mini and Qwen2.5-Coder-32B. We also observe a regime shift around the \$18.3 mark as Figure \ref{fig:combined_perf_vs_cost} shows. Below this threshold, O3 + Qwen32B performs best, whereas above it, O4 + GPT-4o-mini becomes more cost-effective.

These results suggest that no method is universally optimal. Instead, the best strategy depends on the deployment scenario, specifically the available budget and required performance. This leads to one of our key actionable contributions: \textit{effective strong–weak collaboration requires choosing methods that are conditioned on budget and accuracy constraints}. 
Taken together, our findings suggest a set of actionable principles for method selection. (1) Purely weak model-based approaches are inefficient overall, wherein spending as much on a weak model as one would on a strong model yields lower performance for the same cost; (2) Context-based augmentation is often less effective than pipeline-based methods, i.e. when budget allows, it is more efficient to actively involve the strong model. (3) In low-budget settings, strategies like \textit{Weak LM First} or \textit{Weak Router} offer strong efficiency by limiting strong LM usage. (4) In higher-budget regimes, pipelines like \textit{Strong LM First} can approach strong model performance at substantially reduced cost. These principles offer practical guidance for selecting collaboration strategies that align with real-world cost and performance constraints.


% Across model pairs and cost regimes, we observe that no single collaboration method consistently dominates. Pipeline-based strategies like Strong LM First and Weak LM First generally perform best for their cost, particularly when the weak model is reasonably capable. In contrast, when the weak model is very underpowered, such as Qwen2.5-Coder-7B, even collaborative setups yield modest gains at best. Dynamic approaches like Weak Router strike a strong cost–performance balance, especially with closed-source weak models like GPT-4o-mini.

% The effectiveness of each method also depends heavily on the model pair and budget. For example, Figure \ref{fig:subfig6} shows that Strong LM First with O3-mini and Qwen2.5-Coder-32B achieves nearly the same resolution rate as using O3-mini alone, while costing only 60\% as much. Beyond that point, additional spending delivers little improvement, highlighting the value of targeted collaboration, i.e., using the strong model just enough to offset the weak model’s limitations without overspending. Moreover, figure \ref{fig:combined_perf_vs_cost} shows a shift in optimal configurations around the \$18.3 mark: O3 + Qwen32B dominates below this threshold, while O4 + GPT-4o-mini becomes more effective above it. These trends underscore that \textit{the best strategy depends not only on absolute model strength but also on budget and performance targets}.


\subsection{Interesting cases}

\start{Instance-level help is better than repo-level help}

All static repo-level context methods proved ineffective across model pairs. Techniques like providing a repository summary, high-level structural info, or FAQs consistently failed to improve the weak model’s success rate by any significany amount. We interpret this as evidence that broad high-level context is too abstract to aid in solving specific coding issues. Specifically, the added information likely distracts the weak LM or dilutes the truly relevant file-level details. Similarly, incorporating few-shot examples in the prompt (whether randomly selected issues or semantically similar ones) did not boost performance and instead reduces the weak LM's performance below the base performance. On the other hand, methods under instance-level context, i.e. plan and instance-level QA pairs, were mostly successful across the board. This shows that although such methods are significantly more costly than providing repo-level context, the gain in performance is far greater, thus making such methods generally more efficient.

\start{Weak Router is better than Strong Router.}

A particularly interesting finding is the counter-intuitive performance of our Dynamic Collaboration strategies, where we observe the weak router often outperforming the strong router, both in terms of resolution rate and cost. For instance, we see that in the case with O4-mini as the strong LM and Qwen2.5-Coder-32B as the weak LM, the weak router setting achieves a resolution rate that is 6 percentage points higher, with a 20\% lesser cost. We suspect that this gap might be due to differences in fundamental capabilities of the models we consider as strong or weak. We see that models like O3-mini and O4-mini, inspite of being good at problem solving, end up overthinking when it comes to making decisions like routing \cite{cuadron2025dangeroverthinkingexaminingreasoningaction}. Only in scenarios where the weak model is extremely incapable, such as Qwen2.5-Coder-7B, did we see the strong router edge out slightly in success rate, and even there the gains were marginal, suggesting it’s rarely worth the cost.

\start{Prompt Reduction trades turn-wise validity for overall performance}

Another notable finding involves the Prompt Reduction strategy, which involves using the weak LM first to get rid of irrelevant context before using the strong LM for generation. Surprisingly, this leads to a significantly lower valid patch rate (~65\% as compared to ~95\% on average for other successful methods), increasing the number of retries and inflating cost. Despite this, prompt reduction often yielded better resolution rates than settings with full prompt context. This counterintuitive result suggests that aggressively trimming irrelevant or distracting files can help the model focus on essential components, even if many attempts fail in the process. In effect, prompt reduction trades off per-attempt quality for increased focus, leading to higher success at the cost of efficiency. However, this strategy can be expensive and unreliable when budget is limited or when model validity is highly sensitive to missing context.

% Principles for choosing models / methods given cost and performance constraints. What are our 'actionable' contributions?
